Learning Discrete Concepts in Latent Hierarchical Models

Learning concepts from natural high-dimensional data (e.g., images) holds potential in building human-aligned and interpretable machine learning models. Despite its encouraging prospect, formalization and theoretical insights into this crucial task are still lacking. In this work, we formalize concepts as discrete latent causal variables that are related via a hierarchical causal model that encodes different abstraction levels of concepts embedded in high-dimensional data (e.g., a dog breed and its eye shapes in natural images). We formulate conditions to facilitate the identification of the proposed causal model, which reveals when learning such concepts from unsupervised data is possible. Our conditions permit complex causal hierarchical structures beyond latent trees and multi-level directed acyclic graphs in prior work and can handle high-dimensional, continuous observed variables, which is well-suited for unstructured data modalities such as images. We substantiate our theoretical claims with synthetic data experiments. Further, we discuss our theory's implications for understanding the underlying mechanisms of latent diffusion models and provide corresponding empirical evidence for our theoretical insights.

==> sections/methods.tex <==


% \section{Algorithms: Generative VQ-VAE}


% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=.66\textwidth]{figures/vq_vae.png}
% %     \caption{\textbf{VQ-VAE with a continuous latent subspace.} }
% %     \label{fig:generative_vq_vae}
% % \end{figure}



% \begin{itemize}
%     \item Our encoder directly maps $\xx$ to the highest level discrete variable $\zdd{(L)}$ (binary variables) as in \citet{wang2023binary}.
%     \item The hierarchical structure (sparsity) is entailed in the decoding phase: we train an UNeT with level index conditioning and sparsity constraints and apply it multiple times to $\zdd{(L)}$ to ideally descend to $ \zdd{(1)} $. Then, the decoder in \citet{wang2023binary} introduces the continuous information and maps $\zdd{(L)}$ to $\xx$.
%     \item The decoder architecture could assume a sparse attention model~\citep{hassani2023neighborhood} and we interpret the layer outputs as the latent variables (we do need to binarize them, though).
%     \item We employ the binary diffusion process~\citep{wang2023binary} to the top level discrete variable $\zdd{(L)}$ as its prior distribution for sampling novel samples.
%     \item Because we don't know the number of levels in the true model, the encoder's output may not be the top level. We apply diffusion to sample directly from a middle level and set the number of levels from the bottom with the decoder architecture.
% \end{itemize}



% \begin{itemize}
%     \item Offline training with individual VQVAE losses.
%     \item Offline training with individual VQGAN losses.
%     \item Sequential training.
%     \item LSGM + hierarchical VAE literature - online.
% \end{itemize}

% Routes for the empirical section:
% \begin{itemize}
%     \item Hierarchical models:
%     \begin{itemize}
%         \item Composition: 
%         \begin{itemize}
%             \item Each level retains a fraction of the channels.
%             \item Each level entails spatial compression (sparsity).
%             \item Only one quantization for each latent variable.
%         \end{itemize}
%         \item Expected outcomes:
%         \begin{itemize}
%             \item The generation quality companion over hierarchical levels.
%             \item Interventions on disparate levels yield distinct shifts.
%         \end{itemize}
%     \end{itemize}

%     \item Understand the binary diffusion models as a hierarchical model:
%     \begin{itemize}
%         \item Show that low levels correspond to local features (with the tools from \citet{park2023understanding}).
%         \item Impose sparsity constraints to view the disentanglement.
%     \end{itemize}
% \end{itemize}

% - Local channel splitting.
% - Partial quantization.
% - Downsampling.
% - Channel merging at the decoder.
% - Consider full feature maps and a concatenated diffusion model.
% - Separate diffusions.
